Model-Free Approaches to Discern Non-Stationary Microstructure Noise and Time-Varying Liquidity in High-Frequency Data

In this paper, we provide non-parametric statistical tools to test stationarity of microstructure noise in general hidden Ito semimartingales, and discuss how to measure liquidity risk using high frequency financial data. In particular, we investigate the impact of non-stationary microstructure noise on some volatility estimators, and design three complementary tests by exploiting edge effects, information aggregation of local estimates and high-frequency asymptotic approximation. The asymptotic distributions of these tests are available under both stationary and non-stationary assumptions, thereby enable us to conservatively control type-I errors and meanwhile ensure the proposed tests enjoy the asymptotically optimal statistical power. Besides it also enables us to empirically measure aggregate liquidity risks by these test statistics. As byproducts, functional dependence and endogenous microstructure noise are briefly discussed. Simulation with a realistic configuration corroborates our theoretical results, and our empirical study indicates the prevalence of non-stationary microstructure noise in New York Stock Exchange.

==> V-nonStationary.tex <==
\subsection{$V(Y,K_n,s_n,2)^n$ in the presence of non-stationary noises}
%Although we have found the asymptotic distribution of the test statistic under the null hypothesis (when the noise process is stationary), we should investigate the behavior of the second test statistic $V(Y,K,2)^n_T$ under the alternative hypothesis.
Below, we use a heuristic argument to look at the behavior of the test statistic under non-stationary noise.

By (\ref{tsdif2}), we know for a small time interval $[T_i-\Delta T,T_i+\Delta T]$ which contains large amount of observations, namely $K$ observations, we have:
\begin{eqnarray*}
N(Y,K)_{[T_i-\Delta T,T_i+\Delta T]}&\approx&\text{Asym. Gaussian Martingales}\\
&+&\sqrt{K}\left[g_{T_i-\Delta T}(\omega^{(0)}))-\frac{1}{2\Delta T}\int_{T_i-\Delta T}^{T_i+\Delta T}g_t(\omega^{(0)})\mathrm{d}t+g_{T_i+\Delta T}(\omega^{(0)})\right]
\end{eqnarray*}
we assume $g_t(\cdot)$ is a function of $d$ latent variable(s), denoted by $\{f^{(k)}_t(\omega^{(0)})\}_{t\ge 0}$, $k=1,\cdots,d$, and assume $g_t(\cdot)\in \mathcal{C}^2(\mathbb{R}^d)$ with nonzero second-order derivative for each $t\in [0,T]$ and $g_t(\cdot)$ is differentiable w.r.t. time variable. Besides, assume that for each $k$, $\{f^{(k)}_t(\omega^{(0)})\}_{t\ge 0}$ is also an It\^o process with volatility $\{\sigma_t^{(k)}\}_{t\ge 0}$, and the spot correlation between $f^{(j)}_t(\omega^{(0)})$ and $f^{(k)}_{t+s}(\omega^{(0)})$  is $\rho^{(jk)}_t\mathds{1}_{\{s=0\}}$. In other words, we can write
\begin{equation}
g_t(\omega^{(0)})\equiv g\left(t,\omega^{(0)},f_t^{(1)}(\omega^{(0)}),f_t^{(2)}(\omega^{(0)}),\cdots,f_t^{(d)}(\omega^{(0)})\right)
\end{equation}
also note that
\begin{equation*}
g_{T_i-\Delta T_i}(\omega^{(0)})-2g_{T_i}(\omega^{(0)})+g_{T_i+\Delta T}(\omega^{(0)})=\left(g_{T_i+\Delta T}(\omega^{(0)})-g_{T_i}(\omega^{(0)})\right)-\left(g_{T_i}(\omega^{(0)})-g_{T_i-\Delta T}(\omega^{(0)})\right)
\end{equation*}

When $\Delta T\longrightarrow 0$, by It\^o formula:
\begin{eqnarray*}
%\begin{equation*}
%\begin{array}
g_{T_i+\Delta T}(\omega^{(0)})-g_{T_i}(\omega^{(0)})&\approx&\frac{\partial}{\partial t}g_{T_i}(\omega^{(0)})\Delta T+\sum^d_{k=1}\frac{\partial g_{T_i}(\omega^{(0)})}{\partial f_t^{(k)}(\omega^{(0)})}\Delta f^{(k)}_{T_i+\Delta T}(\omega^{(0)})\\
&&+\frac{1}{2}\sum^d_{j=1}\sum^d_{k=1}\frac{\partial^2 g_{T_i}(\omega^{(0)})}{\partial f_t^{(j)}(\omega^{(0)})\partial f_t^{(k)}(\omega^{(0)})}\rho^{(jk)}_{T_i}\sigma^{(j)}_{T_i}\sigma^{(k)}_{T_i}\Delta T\\
g_{T_i}(\omega^{(0)})-g_{T_i-\Delta T}(\omega^{(0)})&\approx&\frac{\partial}{\partial t}g_{T_i}(\omega^{(0)})\Delta T+\sum^d_{k=1}\frac{\partial g_{T_i}(\omega^{(0)})}{\partial f_t^{(k)}(\omega^{(0)})}\Delta f^{(k)}_{T_i}(\omega^{(0)})\\
&&+\frac{1}{2}\sum^d_{j=1}\sum^d_{k=1}\frac{\partial^2 g_{T_i}(\omega^{(0)})}{\partial f_t^{(j)}(\omega^{(0)})\partial f_t^{(k)}(\omega^{(0)})}\rho^{(jk)}_{T_i}\sigma^{(j)}_{T_i}\sigma^{(k)}_{T_i}\Delta T
%\end{array}\right.
%\end{equation*}
\end{eqnarray*}
where $\Delta f^{(k)}_{T_i+\Delta T}(\omega^{(0)})=f^{(k)}_{T_i+\Delta T}(\omega^{(0)})-f^{(k)}_{T_i}(\omega^{(0)})$ and $\Delta f^{(k)}_{T_i}(\omega^{(0)})=f^{(k)}_{T_i}(\omega^{(0)})-f^{(k)}_{T_i-\Delta T}(\omega^{(0)})$, so
\begin{equation*}
g_{T_i-\Delta T}(\omega^{(0)})-2g_{T_i}(\omega^{(0)})+g_{T_i+\Delta T}(\omega^{(0)})\approx\sum^d_{k=1} \frac{\partial g_{T_i}(\omega^{(0)})}{\partial f^{(k)}_t(\omega^{(k)})}\left(\Delta f^{(k)}_{T_i+\Delta T}(\omega^{(0)})-\Delta f^{(k)}_{T_i}(\omega^{(0)})\right)
\end{equation*}
$\left[g_{T_i-\Delta T}(\omega^{(0)})-2g_{T_i}(\omega^{(0)})+g_{T_i+\Delta T}(\omega^{(0)})\right]^2\approx\text{(mean-0 martingale)}+$
\begin{eqnarray*}
&&\sum^d_{j=1}\sum^d_{j=1}\frac{\partial g_{T_i}(\omega^{(0)})}{\partial f^{(j)}_t(\omega^{(0)})}\frac{\partial g_{T_i}(\omega^{(0)})}{\partial f^{(k)}_t(\omega^{(0)})}\left(\Delta f^{(j)}_{T_i}(\omega^{(0)})\cdot\Delta f^{(k)}_{T_i}(\omega^{(0)})\right)\\
&&+\sum^d_{j=1}\sum^d_{j=1}\frac{\partial g_{T_i}(\omega^{(0)})}{\partial f^{(j)}_t(\omega^{(0)})}\frac{\partial g_{T_i}(\omega^{(0)})}{\partial f^{(k)}_t(\omega^{(0)})}\left(\Delta f^{(j)}_{T_i+\Delta T}(\omega^{(0)})\cdot\Delta f^{(k)}_{T_i+\Delta T}(\omega^{(0)})\right)
\end{eqnarray*}

Therefore, under the alternative our test statistic $V(Y,K,2)^n_\mathcal{T}$ behaves like
\begin{eqnarray*}
V(Y,K,2)^n_\mathcal{T}&=&\frac{1}{r_n-s_n+1}\sum_{T_i}\left|N(Y,K)_{[T_i-\Delta T,T_i+\Delta T]}\right|^2\\
&\approx&(\text{Martingales}) + (\text{average of Asym. Chi-squares})\\
&&+\frac{2K}{\mathcal{T}}\left[\sum^d_{j=1}\sum^d_{k=1}\int^T_{0}\frac{\partial g_t(\omega^{(0)})}{\partial f_t^{(j)}(\omega^{(0)})}\frac{\partial g_t(\omega^{(0)})}{\partial f_t^{(k)}(\omega^{(0)})}\rho^{(jk)}_t\sigma^{(j)}_t\sigma^{(k)}_t\mathrm{d}t\right]
\end{eqnarray*}

% the test, if we set $r_n=o(K)$,
Based on this finding, the second test statistic will explode under non-stationary microstructure noise, and in this situation, this test can easily distinguish non-stationary noise.

